VerilogMonkey: Exploring Parallel Scaling for Automated Verilog Code Generation with LLMs

We present VerilogMonkey, an empirical study of parallel scaling for the under-explored task of automated Verilog generation. Parallel scaling improves LLM performance by sampling many outputs in parallel. Across multiple benchmarks and mainstream LLMs, we find that scaling to hundreds of samples is cost-effective in both time and money and, even without any additional enhancements such as post-training or agentic methods, surpasses prior results on LLM-based Verilog generation. We further dissect why parallel scaling delivers these gains and show how output randomness in LLMs affects its effectiveness.

==> chapters/Nan/performance_table.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}


% VerilogEval, Pass@1: 80.13%, Pass@5: 89.10%, Pass@10: 92.31%, Pass@all: 94.23%
% RTLLM: Version: claude37sonnet-thinking, Pass@1: 68.00%, Pass@5: 78.00%, Pass@10: 78.00%, Pass@all: 78.00%
% GenBen: Version: claude37sonnet-thinking, Pass@1: 45.88%, Pass@5: 48.24%, Pass@10: 48.24%, Pass@all: 48.24%


\begin{table*}
\centering
\caption{\oursys's performance across benchmarks and its comparison with baselines.
}
\label{tab:performance-cmp-baseline-verilogeval}
\renewcommand{\arraystretch}{1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccc}
%%%%%%%%%%
\Xhline{1.1pt}
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Baseline}}} & \multicolumn{3}{c}{\textbf{VerilogEval (\%)}} \\ \cline{3-5} 
\multicolumn{2}{c}{} & Pass@$1$ & Pass@$5$ & Pass@$10$ \\ 
\hline \hline
%%%%%%%%
\multicolumn{5}{c}{} \\ \hline 
 %
 \multicolumn{2}{c}{CraftRTL~\cite{liu2024craftrtl}} &68.00  & 72.40 &  74.60\\
\multicolumn{2}{c}{OriGen~\cite{origen} } & 51.40 & 58.60 & 62.20 \\
\multicolumn{2}{c}{AutoVCoder~\cite{autovcoder}} & 48.50 & 55.90 & - \\
\multicolumn{2}{c}{CodeV~\cite{codev}} & 53.20 & 65.10 & 68.50 \\
% \multicolumn{2}{c}{RTL-Coder~\cite{rtlcoder}} & 37.50 & 50.50 & 55.50 \\
\multicolumn{2}{c}{VerilogCoder~\cite{ho2024verilogcoder}} &\cellcolor{silver!40}\textbf{94.20} &-&- \\
\hline
%%%%% 
\multicolumn{5}{c}{} \\ \hline
%
\multicolumn{2}{c}{OpenAI o3-mini} & 81.41 & 89.10 & 89.10 \\
\multicolumn{2}{c}{OpenAI o1} & 74.36 & 85.90 & 85.90 \\ 
\multicolumn{2}{c}{Gemini-2.5-pro} & 76.92 & 90.38 & 90.38 \\ 
\multicolumn{2}{c}{Claude-3.7-Sonnet-Think} & 80.13 & 89.10 & 92.31 \\ 
\Xhline{1.1pt}
%%%%%%
\multicolumn{2}{c}{\textbf{\oursys}} & Hit@$1$ & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Hit@$512$\\ (Improvement)\end{tabular}} \\ \hline \hline
%
\multicolumn{2}{c}{Gemini-1.5-flash} & 44.87 & \multicolumn{2}{c}{56.41 (+11.54)} \\
\multicolumn{2}{c}{Gemini-2.0-flash} & 61.54 & \multicolumn{2}{c}{82.05 (+20.51)} \\
\multicolumn{2}{c}{GPT-4o-mini} & 54.49 & \multicolumn{2}{c}{76.92 (+22.43)} \\
\multicolumn{2}{c}{GPT-4o} & 64.10 & \multicolumn{2}{c}{\cellcolor{gold!40}87.18 (+23.08)} \\
\multicolumn{2}{c}{Claude-3.5-Haiku} & 57.05 & \multicolumn{2}{c}{80.77 (+23.72)} \\ 
\multicolumn{2}{c}{Claude-3.7-Sonnet} & 75.00 & \multicolumn{2}{c}{\cellcolor{gold!60}\textbf{94.87 (+19.87)}} \\
\Xhline{1.1pt}
\end{tabular}%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{tabular}{ccccc}
%%%%%%%%%%
\Xhline{1.1pt}
\multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{\textbf{RTLLM v2 (\%)}} \\ \cline{3-5} 
\multicolumn{2}{c}{} & Pass@$1$ & Pass@$5$ & Pass@$10$ \\ 
\hline \hline
%%%%%%%%
\multicolumn{5}{c}{\textit{Existing Work} *} \\ \hline 
 %
 \multicolumn{2}{c}{HDLCORE~\cite{ping2025hdlcore}} &60.00 &62.00 &- \\
 \cline{1-5}
\multicolumn{5}{c}{\textbf{RTLLM v1 (\%)} **}  \\
\cline{1-5}
\multicolumn{2}{c}{CraftRTL~\cite{liu2024craftrtl}} & 49.00 & 65.80 & 74.50 \\
\multicolumn{2}{c}{OriGen~\cite{origen}} & - & 65.50 & - \\
\multicolumn{2}{c}{CodeV~\cite{codev}} & 36.60 & 53.30 & 61.30 \\
\hline
%%%%% 
\multicolumn{5}{c}{\textit{Reasoning Models}} \\ \hline
%
\multicolumn{2}{c}{} & 72.00 & 78.00 & 78.00 \\
\multicolumn{2}{c}{} & 64.00 & 76.00 & 78.00 \\ 
\multicolumn{2}{c}{} & 70.00 & 78.00 & \cellcolor{silver!40}\textbf{80.00} \\ 
\multicolumn{2}{c}{} & 68.00 & 78.00 & 78.00 \\ 
\Xhline{1.1pt}
%%%%%%
\multicolumn{2}{c}{} & Hit@$1$ & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Hit@$512$\\ (Improvement)\end{tabular}} \\ \hline \hline
%
\multicolumn{2}{c}{} & 56.00 & \multicolumn{2}{c}{72.00 (+16.00)} \\
\multicolumn{2}{c}{} & 60.00 & \multicolumn{2}{c}{\cellcolor{gold!60}\textbf{84.00 (+24.00)}} \\
\multicolumn{2}{c}{} & 64.00 & \multicolumn{2}{c}{80.00 (+16.00)} \\
\multicolumn{2}{c}{} & 60.00 & \multicolumn{2}{c}{\cellcolor{gold!40}82.00 (+22.00)} \\
\multicolumn{2}{c}{} & 62.00 & \multicolumn{2}{c}{80.00 (+18.00)} \\ 
\multicolumn{2}{c}{} & 70.00 & \multicolumn{2}{c}{\cellcolor{gold!60}\textbf{84.00 (+14.00)}} \\
\Xhline{1.1pt}
\end{tabular}%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{tabular}{ccccc}
%%%%%%%%%%
\Xhline{1.1pt}
\multicolumn{2}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{\textbf{GenBen (\%)} ***} \\ \cline{3-5} 
\multicolumn{2}{c}{} & Pass@$1$ & Pass@$5$ & Pass@$10$ \\ 
\hline \hline
%%%%%%%%
\multicolumn{5}{c}{} \\ \hline 
 %
\multicolumn{2}{c}{GPT-3.5-Turbo} & - & 26.70 & - \\
\multicolumn{2}{c}{QWEN-v1-max} & - & 21.20 &- \\
\multicolumn{2}{c}{GLM-4v-plus} & - & 7.50 & - \\
 \multicolumn{2}{c}{Llama3} &- & 6.90 & -\\
\multicolumn{2}{c}{-} &  & &  \\
\hline
%%%%% 
\multicolumn{5}{c}{} \\ \hline
%
\multicolumn{2}{c}{} & 44.71 & 47.06 & 47.06  \\
\multicolumn{2}{c}{} & 43.53 & 47.06 & 47.06 \\ 
\multicolumn{2}{c}{} & 45.88 & 47.06 & 47.06  \\ 
\multicolumn{2}{c}{} & 45.88 & 48.24 & \cellcolor{silver!40}\textbf{48.24}  \\ 
\Xhline{1.1pt}
%%%%%%
\multicolumn{2}{c}{} & Hit@$1$ & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Hit@$512$\\ (Improvement)\end{tabular}} \\ \hline \hline
%
\multicolumn{2}{c}{} & 42.35 & \multicolumn{2}{c}{47.06 (+4.71)} \\
\multicolumn{2}{c}{} & 41.18 & \multicolumn{2}{c}{50.59 (+9.41)} \\
\multicolumn{2}{c}{} & 40.00 & \multicolumn{2}{c}{\cellcolor{gold!60}\textbf{55.29 (+15.29)}} \\
\multicolumn{2}{c}{} & 44.71 & \multicolumn{2}{c}{\cellcolor{gold!60}\textbf{55.29 (+10.58)}} \\
\multicolumn{2}{c}{} & 44.71 & \multicolumn{2}{c}{51.76 (+7.05)} \\ 
\multicolumn{2}{c}{} & 48.24 & \multicolumn{2}{c}{\cellcolor{gold!40}54.12 (+5.88)} \\
\Xhline{1.1pt}
\end{tabular}%
%
}

\begin{tabular}{p{0.97\linewidth}}
\textbf{\dag}\ \oursys's top-2 performances are highlighted in yellow. Best performances in baselines on each benchmark are highlighted in gray. \\
\textbf{*} Data for the Existing Work is directly sourced from the corresponding papers. ``-'' indicates unavailable or not reported. 
% \textbf{**} RTLLM has v1 and v2 versions. Compared to v1, v2 has refined the specifications and added some new problems. 
% Several early studies were conducted using v1, so direct comparisons are not feasible. Still, we provide their performances on v1 as a reference. 
\end{tabular}
\end{table*}




